Technical Report: Sensor-Based Reactive Symbolic Planning in Partially Known Environments

This paper considers the problem of completing assemblies of passive objects in nonconvex environments, cluttered with convex obstacles of unknown position, shape and size that satisfy a specific separation assumption. A differential drive robot equipped with a gripper and a LIDAR sensor, capable of perceiving its environment only locally, is used to position the passive objects in a desired configuration. The method combines the virtues of a deliberative planner generating high-level, symbolic commands, with the formal guarantees of convergence and obstacle avoidance of a reactive planner that requires little onboard computation and is used online. The validity of the proposed method is verified both with formal proofs and numerical simulations.

==> Makefile <==
#
#  Makefile for automating LaTeX related tasks and administrating a 
#  directory of numerous thesis-related files.
#
#  Prepared by Neil C. Miller
#  Modifed by Lord Simon Cuce III
#  May, 1997
#
#  Revision 2.0 5/12/97
#

INCLUDEFILES = 

	FILENAME = body
	ARCHIVE = backup
	PAPERTYPE = a4

.DEFAULT:
	@echo Sorry, that is an undefined target.

help:
	@echo
	@echo Help for make utility:
	@echo
	@echo   make	    - shows this help.
	@echo   make dvi	- executes latex one time.
	@echo   make clean      - removes all backup and output files.
	@echo   make ps	 - executes dvips one time.
	@echo   make bib	- executes bibtex one time.
	@echo   make all	- runs latex several times, bibtex and dvips.
	@echo   make backup     - creates a .tar.gz backup of all files.
	@echo
	@echo Filenames for the main document and backup archive are 
	@echo specified in the Makefile.
	@echo

%:	
	@echo "$@" | latex $(FILENAME) 

dvi:
	@echo $(INCLUDEFILES)  | latex $(FILENAME)

clean:
	@$(RM) *% *.bak *.dvi $(FILENAME).ps

realclean:
	@$(RM) *% *.bak *.dvi $(FILENAME).ps *.aux *.bbl *.blg *.ilg *.ind *.lof *.log *.lot *.lof *.toc *.loa *~

ps:
	@dvips -G0 -R0 -t$(PAPERTYPE) -o $(FILENAME).ps $(FILENAME)
goodps:
	@dvips -G0 -Ppdf -R0 -t$(PAPERTYPE) -o $(FILENAME).ps $(FILENAME)

pdf:
	dvips -G0 -Ppdf -R0 -t$(PAPERTYPE) -o tmp.ps $(FILENAME)
	ps2pdf -dCompatibilityLevel=1.4 -dMAxSubsetPct=100 -dSubsetFonts=true -dEmbedAllFonts=true -sPAPERSIZE=$(PAPERTYPE) tmp.ps $(FILENAME).pdf
	$(RM) -f tmp.ps

bib:
	@bibtex $(FILENAME)

# This doesn't work perfectly.  For example, the changing of a section
# name does not cause a Warning, even though its change will not be 
# reflected in the TOC until the next pass.  So, "all" should be done 
# after "realclean" before final submission.  Possibly a good use for a 
# small perl script which checks to see that the TOC is up-to-date.
all:
	echo '** Running LaTeX **'
	echo $(INCLUDEFILES) | latex $(FILENAME);
	@if ( grep "There were undefined references"        \
			$(FILENAME).log >/dev/null ); then  \
		echo '** Running BibTeX **';                \
		bibtex $(FILENAME);                         \
		echo '** Re-running LaTeX **';              \
		echo $(INCLUDEFILES) | latex $(FILENAME);  \
	fi
	@while ( grep "Rerun to get cross-references"       \
			$(FILENAME).log >/dev/null ); do    \
		echo '** Re-running LaTeX **';              \
		echo $(INCLUDEFILES) | latex $(FILENAME);  \
	done

oldall:
	@latex $(FILENAME)
	@bibtex $(FILENAME)
	@latex $(FILENAME)
	@latex $(FILENAME)

allps: all
	@dvips -G0 -Ppdf -o $(FILENAME).ps $(FILENAME)

backup:
	@$(RM) $(ARCHIVE).tar.gz
	@tar cf $(ARCHIVE).tar *
	@gzip $(ARCHIVE).tar
	@ls -l $(ARCHIVE).tar.gz


